From Exoplanets to Quasars: Adventures in Angular Differential Imaging

Angular differential imaging provides a novel way of probing the high contrast of our universe. Until now, its applications have been primarily localized to searching for exoplanets around nearby stars. This work presents a suite of applications of angular differential imaging from the theoretical underpinning of data reduction, to its use characterizing substellar objects to a new application looking for the host galaxies of damped Lyman {\alpha} systems, which are usually lost in the glare of ultra-bright quasars along the line of sight.

==> macros/initial_commands.tex <==
% These commands are used
% immediate after \begin{document}

% Setup old style numerals macro
\newcommand\osn[1]{\oldstylenums{#1}\xspace}

% Setup a definition style macro
\newcommand\defn[1]{\textbf{#1}}

